On a theorem of B. Keller on Yoneda algebras of simple modules

A theorem of Keller states that the Yoneda algebra of the simple modules over a finite-dimensional algebra is generated in cohomological degrees $0$ and $1$ as a minimal $A_\infty$-algebra. We provide a proof of an extension of Keller's theorem to abelian length categories by reducing the problem to a particular class of Nakayama algebras, where the claim can be shown by direct computation.

==> ar-quiver.tex <==
\begin{resizebox}{\textwidth}{!}{%
    \begin{tikzpicture}[rotate=-45]
      \node (000) at (0,0) {$S_a$};%
      \node (001) at (0,1) {$\bullet$};%
      \node (002) at (0,2) {$\bullet$};%
      \node (003) at (0,3) {$\bullet$};%
      \node (004) at (0,4) {$\bullet$};%
      \node (005) at (0,5) {$M_1$};
      \draw[>->] (000)--(001);%
      \draw[>->] (001)--(002);%
      \draw[>->] (002)--(003);%
      \draw[>->] (003)--(004);%
      \draw[>->] (004)--(005);%
      \begin{scope}[shift={(1,1)}]
        \node (100) at (0,0) {$\bullet$};%
        \node (101) at (0,1) {$\bullet$};%
        \node (102) at (0,2) {$\bullet$};%
        \node (103) at (0,3) {$\bullet$};%
        \node (104) at (0,4) {$N_1$};%
        \node (105) at (0,5) {$\bullet$};%
        \node (106) at (0,6) {$\bullet$};%
        \node (107) at (0,7) {$\bullet$};%
        \node (108) at (0,8) {$\bullet$};%
        \node (109) at (0,9) {$\bullet$};%
        \node (1010) at (0,10) {$M_2$};%
        \draw[>->] (100)--(101);%
        \draw[>->] (101)--(102);%
        \draw[>->] (102)--(103);%
        \draw[>->] (103)--(104);%
        \draw[>->] (104)--(105);%
        \draw[>->] (105)--(106);%
        \draw[>->] (106)--(107);%
        \draw[>->] (107)--(108);%
        \draw[>->] (108)--(109);%
        \draw[>->] (109)--(1010);%
      \end{scope}
      \begin{scope}[shift={(2,2)}]
        \node (200) at (0,0) {$\bullet$};%
        \node (201) at (0,1) {$\bullet$};%
        \node (202) at (0,2) {$\bullet$};%
        \node (203) at (0,3) {$\bullet$};%
        \node (204) at (0,4) {$\bullet$};%
        \node (205) at (0,5) {$\bullet$};%
        \node (206) at (0,6) {$\bullet$};%
        \node (207) at (0,7) {$\bullet$};%
        \node (208) at (0,8) {$\bullet$};%
        \node (209) at (0,9) {$\bullet$};%
        \draw[>->] (200)--(201);%
        \draw[>->] (201)--(202);%
        \draw[>->] (202)--(203);%
        \draw[>->] (203)--(204);%
        \draw[>->] (204)--(205);%
        \draw[>->] (205)--(206);%
        \draw[>->] (206)--(207);%
        \draw[>->] (207)--(208);%
        \draw[>->] (208)--(209);%
      \end{scope}
      \begin{scope}[shift={(3,3)}]
        \node (300) at (0,0) {$\bullet$};%
        \node (301) at (0,1) {$\bullet$};%
        \node (302) at (0,2) {$\bullet$};%
        \node (303) at (0,3) {$\bullet$};%
        \node (304) at (0,4) {$\bullet$};%
        \node (305) at (0,5) {$\bullet$};%
        \node (306) at (0,6) {$\bullet$};%
        \node (307) at (0,7) {$\bullet$};%
        \node (308) at (0,8) {$\bullet$};%
        \draw[>->] (300)--(301);%
        \draw[>->] (301)--(302);%
        \draw[>->] (302)--(303);%
        \draw[>->] (303)--(304);%
        \draw[>->] (304)--(305);%
        \draw[>->] (305)--(306);%
        \draw[>->] (306)--(307);%
        \draw[>->] (307)--(308);%
      \end{scope}
      \begin{scope}[shift={(4,4)}]
        \node (400) at (0,0) {$\bullet$};%
        \node (401) at (0,1) {$\bullet$};%
        \node (402) at (0,2) {$\bullet$};%
        \node (403) at (0,3) {$\bullet$};%
        \node (404) at (0,4) {$\bullet$};%
        \node (405) at (0,5) {$\bullet$};%
        \node (406) at (0,6) {$\bullet$};%
        \node (407) at (0,7) {$\bullet$};%
        \draw[>->] (400)--(401);%
        \draw[>->] (401)--(402);%
        \draw[>->] (402)--(403);%
        \draw[>->] (403)--(404);%
        \draw[>->] (404)--(405);%
        \draw[>->] (405)--(406);%
        \draw[>->] (406)--(407);%
      \end{scope}
      \begin{scope}[shift={(5,5)}]
        \node (500) at (0,0) {$S_c$};%
        \node (501) at (0,1) {$\bullet$};%
        \node (502) at (0,2) {$\bullet$};%
        \node (503) at (0,3) {$\bullet$};%
        \node (504) at (0,4) {$\bullet$};%
        \node (505) at (0,5) {$\bullet$};%
        \node (506) at (0,6) {$M_2'$};%
        \draw[>->] (500)--(501);%
        \draw[>->] (501)--(502);%
        \draw[>->] (502)--(503);%
        \draw[>->] (503)--(504);%
        \draw[>->] (504)--(505);%
        \draw[>->] (505)--(506);%
      \end{scope}
      \begin{scope}[shift={(6,6)}]
        \node (600) at (0,0) {$\bullet$};%
        \node (601) at (0,1) {$\bullet$};%
        \node (602) at (0,2) {$\bullet$};%
        \node (603) at (0,3) {$\bullet$};%
        \node (604) at (0,4) {$\bullet$};%
        \node (605) at (0,5) {$N_2$};%
        \node (606) at (0,6) {$\bullet$};%
        \node (607) at (0,7) {$\bullet$};%
        \node (608) at (0,8) {$\bullet$};%
        \node (609) at (0,9) {$\bullet$};%
        \node (6010) at (0,10) {$\cdots$};%
        \draw[>->] (600)--(601);%
        \draw[>->] (601)--(602);%
        \draw[>->] (602)--(603);%
        \draw[>->] (603)--(604);%
        \draw[>->] (604)--(605);%
        \draw[>->] (605)--(606);%
        \draw[>->] (606)--(607);%
        \draw[>->] (607)--(608);%
        \draw[>->] (608)--(609);%
        \draw[>->] (609)--(6010);%
      \end{scope}
      \begin{scope}[shift={(7,7)}]
        \node (700) at (0,0) {$\bullet$};%
        \node (701) at (0,1) {$\bullet$};%
        \node (702) at (0,2) {$\bullet$};%
        \node (703) at (0,3) {$\bullet$};%
        \node (704) at (0,4) {$\bullet$};%
        \node (705) at (0,5) {$\bullet$};%
        \node (706) at (0,6) {$\bullet$};%
        \node (707) at (0,7) {$\bullet$};%
        \node (708) at (0,8) {$\cdots$};%
        \node (709) at (0,9) {$\bullet$};%
        \draw[>->] (700)--(701);%
        \draw[>->] (701)--(702);%
        \draw[>->] (702)--(703);%
        \draw[>->] (703)--(704);%
        \draw[>->] (704)--(705);%
        \draw[>->] (705)--(706);%
        \draw[>->] (706)--(707);%
        \draw[>->] (707)--(708);%
        \draw[>->] (708)--(709);%
      \end{scope}
      \begin{scope}[shift={(8,8)}]
        \node (800) at (0,0) {$\bullet$};%
        \node (801) at (0,1) {$\bullet$};%
        \node (802) at (0,2) {$\bullet$};%
        \node (803) at (0,3) {$\bullet$};%
        \node (804) at (0,4) {$\bullet$};%
        \node (805) at (0,5) {$\bullet$};%
        \node (806) at (0,6) {$\cdots$};%
        \node (807) at (0,7) {$\bullet$};%
        \node (808) at (0,8) {$\bullet$};%
        \draw[>->] (800)--(801);%
        \draw[>->] (801)--(802);%
        \draw[>->] (802)--(803);%
        \draw[>->] (803)--(804);%
        \draw[>->] (804)--(805);%
        \draw[>->] (805)--(806);%
        \draw[>->] (806)--(807);%
        \draw[>->] (807)--(808);%
      \end{scope}
      \begin{scope}[shift={(9,9)}]
        \node (900) at (0,0) {$\bullet$};%
        \node (901) at (0,1) {$\bullet$};%
        \node (902) at (0,2) {$\bullet$};%
        \node (903) at (0,3) {$\bullet$};%
        \node (904) at (0,4) {$\cdots$};%
        \node (905) at (0,5) {$\bullet$};%
        \node (906) at (0,6) {$\bullet$};%
        \node (907) at (0,7) {$\bullet$};%
        \draw[>->] (900)--(901);%
        \draw[>->] (901)--(902);%
        \draw[>->] (902)--(903);%
        \draw[>->] (903)--(904);%
        \draw[>->] (904)--(905);%
        \draw[>->] (905)--(906);%
        \draw[>->] (906)--(907);%
      \end{scope}
      \begin{scope}[shift={(10,10)}]
        \node (1000) at (0,0) {$\bullet$};%
        \node (1001) at (0,1) {$\bullet$};%
        \node (1002) at (0,2) {$\cdots$};%
        \node (1003) at (0,3) {$\bullet$};%
        \node (1004) at (0,4) {$\bullet$};%
        \node (1005) at (0,5) {$\bullet$};%
        \node (1006) at (0,6) {$\bullet$};%
        \draw[>->] (1000)--(1001);%
        \draw[>->] (1001)--(1002);%
        \draw[>->] (1002)--(1003);%
        \draw[>->] (1003)--(1004);%
        \draw[>->] (1004)--(1005);%
        \draw[>->] (1005)--(1006);%
      \end{scope}
      \begin{scope}[shift={(11,11)}]
        \node (1100) at (0,0) {$\dots$};%
        \node (1101) at (0,1) {$\bullet$};%
        \node (1102) at (0,2) {$\bullet$};%
        \node (1103) at (0,3) {$\bullet$};%
        \node (1104) at (0,4) {$\bullet$};%
        \node (1105) at (0,5) {$\bullet$};%
        \draw[>->] (1100)--(1101);%
        \draw[>->] (1101)--(1102);%
        \draw[>->] (1102)--(1103);%
        \draw[>->] (1103)--(1104);%
        \draw[>->] (1104)--(1105);%
      \end{scope}
      \begin{scope}[shift={(12,12)}]
        \node (1200) at (0,0) {$\bullet$};%
        \node (1201) at (0,1) {$\bullet$};%
        \node (1202) at (0,2) {$\bullet$};%
        \node (1203) at (0,3) {$\bullet$};%
        \node (1204) at (0,4) {$N_d$};%
        \node (1205) at (0,5) {$M_{d+1}$};%
        \draw[>->] (1200)--(1201);%
        \draw[>->] (1201)--(1202);%
        \draw[>->] (1202)--(1203);%
        \draw[>->] (1203)--(1204);%
        \draw[>->] (1204)--(1205);%
      \end{scope}
      \begin{scope}[shift={(13,13)}]
        \node (1300) at (0,0) {$\bullet$};%
        \node (1301) at (0,1) {$\bullet$};%
        \node (1302) at (0,2) {$\bullet$};%
        \node (1303) at (0,3) {$\bullet$};%
        \node (1304) at (0,4) {$\bullet$};%
        \draw[>->] (1300)--(1301);%
        \draw[>->] (1301)--(1302);%
        \draw[>->] (1302)--(1303);%
        \draw[>->] (1303)--(1304);%
      \end{scope}
      \begin{scope}[shift={(14,14)}]
        \node (1400) at (0,0) {$\bullet$};%
        \node (1401) at (0,1) {$\bullet$};%
        \node (1402) at (0,2) {$\bullet$};%
        \node (1403) at (0,3) {$\bullet$};%
        \draw[>->] (1400)--(1401);%
        \draw[>->] (1401)--(1402);%
        \draw[>->] (1402)--(1403);%
      \end{scope}
      \begin{scope}[shift={(15,15)}]
        \node (1500) at (0,0) {$\bullet$};%
        \node (1501) at (0,1) {$\bullet$};%
        \node (1502) at (0,2) {$\bullet$};%
        \draw[>->] (1500)--(1501);%
        \draw[>->] (1501)--(1502);%
      \end{scope} 
      \begin{scope}[shift={(16,16)}]
        \node (1600) at (0,0) {$\bullet$};%
        \node (1601) at (0,1) {$\bullet$};%
        \draw[>->] (1600)--(1601);%
      \end{scope} 
      \begin{scope}[shift={(17,17)}]
        \node (1700) at (0,0) {$S_b$};%
      \end{scope}
      \draw[->>] (001)--(100);%
      \draw[->>] (002)--(101);%
      \draw[->>] (003)--(102);%
      \draw[->>] (004)--(103);%
      \draw[->>] (005)--(104);%
      
      \draw[->>] (101)--(200);%
      \draw[->>] (102)--(201);%
      \draw[->>] (103)--(202);%
      \draw[->>] (104)--(203);%
      \draw[->>] (105)--(204);%
      \draw[->>] (106)--(205);%
      \draw[->>] (107)--(206);%
      \draw[->>] (108)--(207);%
      \draw[->>] (109)--(208);%
      \draw[->>] (1010)--(209);%

      \draw[->>] (201)--(300);%
      \draw[->>] (202)--(301);%
      \draw[->>] (203)--(302);%
      \draw[->>] (204)--(303);%
      \draw[->>] (205)--(304);%
      \draw[->>] (206)--(305);%
      \draw[->>] (207)--(306);%
      \draw[->>] (208)--(307);%
      \draw[->>] (209)--(308);%

      \draw[->>] (301)--(400);%
      \draw[->>] (302)--(401);%
      \draw[->>] (303)--(402);%
      \draw[->>] (304)--(403);%
      \draw[->>] (305)--(404);%
      \draw[->>] (306)--(405);%
      \draw[->>] (307)--(406);%
      \draw[->>] (308)--(407);%

      \draw[->>] (401)--(500);%
      \draw[->>] (402)--(501);%
      \draw[->>] (403)--(502);%
      \draw[->>] (404)--(503);%
      \draw[->>] (405)--(504);%
      \draw[->>] (406)--(505);%
      \draw[->>] (407)--(506);%

      \draw[->>] (501)--(600);%
      \draw[->>] (502)--(601);%
      \draw[->>] (503)--(602);%
      \draw[->>] (504)--(603);%
      \draw[->>] (505)--(604);%
      \draw[->>] (506)--(605);%

      \draw[->>] (601)--(700);%
      \draw[->>] (602)--(701);%
      \draw[->>] (603)--(702);%
      \draw[->>] (604)--(703);%
      \draw[->>] (605)--(704);%
      \draw[->>] (606)--(705);%
      \draw[->>] (607)--(706);%
      \draw[->>] (608)--(707);%
      \draw[->>] (609)--(708);%
      \draw[->>] (6010)--(709);%

      \draw[->>] (701)--(800);%
      \draw[->>] (702)--(801);%
      \draw[->>] (703)--(802);%
      \draw[->>] (704)--(803);%
      \draw[->>] (705)--(804);%
      \draw[->>] (706)--(805);%
      \draw[->>] (707)--(806);%
      \draw[->>] (708)--(807);%
      \draw[->>] (709)--(808);%    

      \draw[->>] (801)--(900);%
      \draw[->>] (802)--(901);%
      \draw[->>] (803)--(902);%
      \draw[->>] (804)--(903);%
      \draw[->>] (805)--(904);%
      \draw[->>] (806)--(905);%
      \draw[->>] (807)--(906);%
      \draw[->>] (808)--(907);%    

      \draw[->>] (901)--(1000);%
      \draw[->>] (902)--(1001);%
      \draw[->>] (903)--(1002);%
      \draw[->>] (904)--(1003);%
      \draw[->>] (905)--(1004);%
      \draw[->>] (906)--(1005);%
      \draw[->>] (907)--(1006);%

      \draw[->>] (1001)--(1100);%
      \draw[->>] (1002)--(1101);%
      \draw[->>] (1003)--(1102);%
      \draw[->>] (1004)--(1103);%
      \draw[->>] (1005)--(1104);%
      \draw[->>] (1006)--(1105);%

      \draw[->>] (1101)--(1200);%
      \draw[->>] (1102)--(1201);%
      \draw[->>] (1103)--(1202);%
      \draw[->>] (1104)--(1203);%
      \draw[->>] (1105)--(1204);%

      \draw[->>] (1201)--(1300);%
      \draw[->>] (1202)--(1301);%
      \draw[->>] (1203)--(1302);%
      \draw[->>] (1204)--(1303);%
      \draw[->>] (1205)--(1304);%

      \draw[->>] (1301)--(1400);%
      \draw[->>] (1302)--(1401);%
      \draw[->>] (1303)--(1402);%
      \draw[->>] (1304)--(1403);%    

      \draw[->>] (1401)--(1500);%
      \draw[->>] (1402)--(1501);%
      \draw[->>] (1403)--(1502);%

      \draw[->>] (1501)--(1600);%
      \draw[->>] (1502)--(1601);%

      \draw[->>] (1601)--(1700);%

      \draw [
      thick,
      decoration={
        brace,
        mirror,
        raise=0.5cm
      },
      decorate
      ] (0,0) -- (5,5) 
      node [pos=0.5,anchor=north,yshift=-0.55cm] {$\ell=\operatorname{len}(M_1)$};
    \end{tikzpicture}
  }%
\end{resizebox}
